Characterizing Service Provider Response to the COVID-19 Pandemic in the United States

The COVID-19 pandemic has resulted in dramatic changes to the daily habits of billions of people. Users increasingly have to rely on home broadband Internet access for work, education, and other activities. These changes have resulted in corresponding changes to Internet traffic patterns. This paper aims to characterize the effects of these changes with respect to Internet service providers in the United States. We study three questions: (1)How did traffic demands change in the United States as a result of the COVID-19 pandemic?; (2)What effects have these changes had on Internet performance?; (3)How did service providers respond to these changes? We study these questions using data from a diverse collection of sources. Our analysis of interconnection data for two large ISPs in the United States shows a 30-60% increase in peak traffic rates in the first quarter of 2020. In particular, we observe traffic downstream peak volumes for a major ISP increase of 13-20% while upstream peaks increased by more than 30%. Further, we observe significant variation in performance across ISPs in conjunction with the traffic volume shifts, with evident latency increases after stay-at-home orders were issued, followed by a stabilization of traffic after April. Finally, we observe that in response to changes in usage, ISPs have aggressively augmented capacity at interconnects, at more than twice the rate of normal capacity augmentation. Similarly, video conferencing applications have increased their network footprint, more than doubling their advertised IP address space.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

\paragraph{Takeaways} 
\begin{itemize}
    \item Utilization increased, latency went higher and then stabilized, 
    throughput remained the same, implying capacity changes and is validated by
    interconnect and IP prefix upgrades. Adding capacity is effective in keeping
    the internet perform well.
    \item Current network infrastructure and provisioning strategies can cope 
    with similar events. Same level of latency increases can be found in other 
    periods of a normal year (such as December).
\end{itemize}

\paragraph{Limitations} 
\begin{itemize}
    \item IP prefix is not a precise reflection of capacity changes
\end{itemize}

\paragraph{Future work} 
\begin{itemize}
    \item More applications and ISPs?
    \item Analysis based on locations.
\end{itemize}

